On the Spectral Efficiency of Multi-user Holographic MIMO Uplink Transmission

With antenna spacing much less than half a wavelength in confined space, holographic multiple-input multiple-output (HMIMO) technology presents a promising frontier in next-generation mobile communication. We delve into the research of the multi-user uplink transmission with both the base station and the users equipped with holographic planar arrays. To begin, we construct an HMIMO channel model utilizing electromagnetic field equations, accompanied by a colored noise model that accounts for both electromagnetic interference and hardware noise. Since this model is continuous, we approximate it within a finite-dimensional space spanned by Fourier space series, which can be defined as the communication mode functions. We show that this channel model samples Green's function in the wavenumber domain in different communication modes. Subsequently, we tackle the challenging task of maximizing the spectral efficiency (SE) of the system, which involves optimizing the continuous current density function (CDF) for each user. Using the aforementioned approximation model, we transform the optimization variables into expansion coefficients of the CDFs on a finite-dimensional space, for which we propose an iterative water-filling algorithm. Simulation results illustrate the efficacy of the proposed algorithm in enhancing the system SE and show the influence of the colored noise and the system parameters on the SE.

==> newcommand.tex <==
%mathcal font
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

%mathbf font
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\be}{\mathbf{e}}
%\newcommand{\bf}{\mathbf{f}}
\newcommand{\bbf}{\mathbf{f}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bi}{\mathbf{i}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bl}{\mathbf{l}}
%\newcommand{\bm}{\mathbf{m}}
\newcommand{\bbm}{\mathbf{m}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}

%rm
\newcommand{\remi}{\mathrm{emi}}
\newcommand{\rhw}{\mathrm{hw}}
\newcommand{\rd}{\mathrm{d}}
\newcommand{\rmax}{\mathrm{max}}
\newcommand{\sinc}{\mathrm{sinc}}
\newcommand{\rrank}{\mathrm{rank}}





%cal font
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbZ}{\mathbb{Z}}



%constant
\newcommand{\emath}{\mathrm{e}}

\newcommand{\hata}{\widehat{a}}
\newcommand{\hath}{\widehat{h}}

\newcommand{\hatba}{\widehat{\ba}}
\newcommand{\hatbg}{\widehat{\bg}}
\newcommand{\hatbh}{\widehat{\bh}}
\newcommand{\hatbx}{\widehat{\bx}}


\newcommand{\hatbG}{\widehat{\bG}}
\newcommand{\hatbH}{\widehat{\bH}}
\newcommand{\hatbQ}{\widehat{\bQ}}
\newcommand{\hatbR}{\widehat{\bR}}

%tilde
\newcommand{\tildeg}{\widetilde{g}}
\newcommand{\tilden}{\widetilde{n}}
\newcommand{\tildey}{\widetilde{y}}
\newcommand{\tildebg}{\widetilde{\bg}}
\newcommand{\tildebh}{\widetilde{\bh}}
\newcommand{\tildebx}{\widetilde{\bx}}
\newcommand{\tildeby}{\widetilde{\by}}
\newcommand{\tildebz}{\widetilde{\bz}}
\newcommand{\tildebD}{\widetilde{\bD}}
\newcommand{\tildebG}{\widetilde{\bG}}
\newcommand{\tildebH}{\widetilde{\bH}}
\newcommand{\tildebQ}{\widetilde{\bQ}}
\newcommand{\tildeDelta}{\widetilde{\Delta}}

%bar
\newcommand{\barg}{\overline{g}}
\newcommand{\barx}{\overline{x}}
\newcommand{\bary}{\overline{y}}
\newcommand{\barz}{\overline{z}}
\newcommand{\barM}{\overline{M}}
\newcommand{\barbg}{\overline{\bg}}
\newcommand{\barbh}{\overline{\bh}}
\newcommand{\barbG}{\overline{\bG}}
\newcommand{\barbr}{\overline{\br}}
\newcommand{\barbx}{\overline{\bx}}
\newcommand{\barby}{\overline{\by}}
\newcommand{\barbz}{\overline{\bz}}
\newcommand{\barbH}{\overline{\bH}}
\newcommand{\barbQ}{\overline{\bQ}}
\newcommand{\barbU}{\overline{\bU}}
\newcommand{\barbarbQ}{\overline{\barbQ}}
\newcommand{\barbOmega}{\overline{\bOmega}}
\newcommand{\barDelta}{\overline{\Delta}}

\newcommand{\barbarbx}{\overline{\barbx}}
\newcommand{\barbarby}{\overline{\barby}}
\newcommand{\barbarbz}{\overline{\barbz}}
\newcommand{\barbarbG}{\overline{\barbG}}

%symbol
\newcommand{\bzero}{\mathbf{0}}
\newcommand{\bone}{\mathbf{1}}
\newcommand{\btwo}{\mathbf{2}}

\newcommand{\btheta}{\boldsymbol\theta}
\newcommand{\bzeta}{\boldsymbol\zeta}
\newcommand{\bSigma}{{\boldsymbol\Sigma}}
\newcommand{\bsigma}{{\boldsymbol\sigma}}
\newcommand{\blambda}{{\boldsymbol\lambda}}
\newcommand{\barblambda}{{\boldsymbol\lambda}}
\newcommand{\bLambda}{{\boldsymbol\Lambda}}
\newcommand{\bOmega}{{\boldsymbol\Omega}}
\newcommand{\bDelta}{{\boldsymbol\Delta}}
\newcommand{\bomega}{{\boldsymbol\omega}}
\newcommand{\bxi}{{\boldsymbol\xi}}
\newcommand{\bXi}{{\boldsymbol\Xi}}
\newcommand{\bPi}{{\boldsymbol\Pi}}
\newcommand{\bPhi}{{\boldsymbol\Phi}}
\newcommand{\brho}{{\boldsymbol\rho}}
\newcommand{\bPsi}{{\boldsymbol\Psi}}
\newcommand{\bpsi}{{\boldsymbol\psi}}
\newcommand{\balpha}{{\boldsymbol\alpha}}
\newcommand{\bkappa}{\boldsymbol{\kappa}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bGamma}{\boldsymbol{\Gamma}}


%special
\newcommand{\bbone}{\mathbbm{1}}
\newcommand{\dr}{\mathrm{d}\mathbf{r}}
\newcommand{\ds}{\mathrm{d}\mathbf{s}}
\newcommand{\rrm}{\mathrm{m}}
\newcommand{\rV}{\mathrm{V}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\alref}[1]{\textbf{Algorithm}~\textbf{\ref{#1}}}
\newcommand{\cororef}[1]{\textit{Corollary}~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\ntb}{\notag\\}
\newcommand{\rsum}{\mathrm{sum}}
\newcommand{\st}{\mathrm{s.t.}}
\newcommand{\oG}{\overline{\bG}}
\newcommand{\qdet}[1]{\det{\bigg|#1\bigg|}}
\newcommand{\rdiag}[1]{\mathrm{diag}\left\{ #1\right\}}
\newcommand{\trace}[1]{\mathrm{tr}\left(#1\right)}
%bb font
\newcommand{\expect}[1]{\mathbb{E}{\left\{#1\right\}}}
% et. al.
\newcommand{\etal}{{\em et al.}}
\newcommand{\ropt}{\mathrm{opt}}
\newcommand{\real}[1]{\Re\{#1\}}
\newcommand{\rect}{\mathrm{rect}}


%Theorem environment
\newtheorem{corollary}{Corollary}
\newtheorem{remark}{Remark}








